Transferable Representation Learning in Vision-and-Language Navigation

Vision-and-Language Navigation (VLN) tasks such as Room-to-Room (R2R) require machine agents to interpret natural language instructions and learn to act in visually realistic environments to achieve navigation goals. The overall task requires competence in several perception problems: successful agents combine spatio-temporal, vision and language understanding to produce appropriate action sequences. Our approach adapts pre-trained vision and language representations to relevant in-domain tasks making them more effective for VLN. Specifically, the representations are adapted to solve both a cross-modal sequence alignment and sequence coherence task. In the sequence alignment task, the model determines whether an instruction corresponds to a sequence of visual frames. In the sequence coherence task, the model determines whether the perceptual sequences are predictive sequentially in the instruction-conditioned latent space. By transferring the domain-adapted representations, we improve competitive agents in R2R as measured by the success rate weighted by path length (SPL) metric.

==> discriminator.tex <==
\section{Multi-modal Sequence Discrimination}
\label{sec:discriminator}

VLN tasks are composed of instruction-path pairs, where a path is a sequence of connected locations along with their corresponding perceptual contexts in some environment. While the end goal of the VLN challenge is to create agents that can follow the navigation instructions, we instead explore an auxiliary task that determines whether an instruction-path pair are a good match for one another. Such discrimination models would be able to align similar concepts in two modalities, \eg, in an instruction like ``\textit{Turn right and move forward around the bed, enter the bathroom and wait there.}'', it is expected that the word \textit{bed} is better aligned with a location on the path that has a bed in the agent's egocentric view. Another reasonable expectation from such models would be to prefer perceptual and language sequences that are predictable and coherent, \eg two successive panoramic sequences that illustrates ``\textit{walk towards TV}'' would align with natural language sequence that describes it.

To this effect, we train a discriminator model that learns to delineate positive instruction-path pairs from negative pairs sampled using different strategies described in Sec.\ref{subsec:discriminator_training}. The discrimination is based on an alignment-based similarity score that determines how well the two input sequences align. This encourages the model to map perceptual and textual signals for final discrimination. Furthermore we introduce an additional noise contrastive estimation (NCE) loss \cite{gutmann:2010:nce} via the CPC framework to model sequence predictability in positive pairs versus incoherent sequences in negative pairs.

\begin{figure}
    \centering
     \includegraphics[clip, width=\linewidth]{imgs/teaser.pdf}
    \qquad
    \scriptsize
    \caption{Overview of the discriminator model structure. Alignment layer corresponds to Eq.\ref{eq:A_compute},\ref{eq:A_softmax},\ref{eq:A_softmin}}

    \label{fig:deoverview}
\end{figure}

\todo{update discriminator model structure to add CPC loss}

\subsection{Model Structure}
\label{subsec:disc_structure}

We use a two-tower architecture \cite{Gillick:2018:DualEncoders,Serban:2018:DualEncoders} as in Fig.~\ref{fig:deoverview} to independently encode the two sequences, with one tower encoding the token sequence $x_1, x_2, ..., x_n$ in the instruction $\mathcal{X}$ and another tower encoding the visual input sequence $v_1, v_2, ..., v_m$ from the path $\mathcal{V}$. Each tower is a bi-directional LSTM \cite{Schuster1997BidirectionalRN} which constructs the latent space representation $H$ of a sequence $i_1, i_2, ..., i_k$ following:

\begin{small}
\begin{align}
    H &= [h_1; h_2; ...; h_k]  \\
    h_t &= \sigma(\overrightarrow{h}_t, \overleftarrow{h}_t)  \\
    \overrightarrow{h}_t &= LSTM(i_t, \overrightarrow{h}_{t-1})  \\
    \overleftarrow{h}_t &= LSTM(i_t, \overleftarrow{h}_{t+1})
\end{align}
\end{small}

\noindent
where $\sigma$ function is used to combine the output of forward and backward LSTM layers.

We denote the latent space representation of instruction $\mathcal{X}$ as $H^X$ and path $\mathcal{V}$ as $H^V$ and compute the alignment-based similarity score as following:

\begin{small}
\begin{align}
    A &= H^X({H^V})^T  \label{eq:A_compute} \\
    \{c\}_{l=1}^{l=X} &= \text{softmax}(A^l) \cdot A^l  \label{eq:A_softmax} \\
    \text{score} &= \text{softmin}(\{c\}_{l=1}^{l=X}) \cdot \{c\}_{l=1}^{l=X}  \label{eq:A_softmin}
\end{align}
\end{small}

\noindent
where $(.)^T$ is matrix transpose transformation, $A$ is the alignment matrix whose dimensions are $[n, m]$ and $A^l$ is the $l$-th row vector in $A$. Eq.\ref{eq:A_softmax} corresponds to taking a softmax along the columns and summing the columns, which amounts to content-based pooling across columns. Then we apply softmin operation along the rows and sum the rows up to get a scalar in Eq.\ref{eq:A_softmin}. Intuitively, optimizing this score encourages the learning algorithm to construct the best worst-case sequence alignment between the two input sequences in latent space.


\subsection{Training}
\label{subsec:discriminator_training}

Training data consists of instruction-path pairs which may be similar (positives) or dissimilar (negatives). The training objective maximizes the log-likelihood of predicting higher alignment-based similarity scores for similar pairs.

We use the human annotated demonstrations in the R2R dataset as our positives and explore three strategies for sampling negatives. For a given instruction-path pair, we sample negatives by keeping the same instruction but altering the path sequence by:

\begin{itemize}
    \item \textit{Path Substitution (PS)} -- randomly picking other paths from the same environment as negatives.
    \item \textit{Partial Reordering (PR)} -- keeping the first and last nodes in the path unaltered and shuffling the intermediate locations of the path.
    \item \textit{Random Walks (RW)} -- sampling random paths of the same length as the original path that either (1) start at the same location and end sufficiently far from the original path or (2) end at the same location and start sufficiently far from the original path.
\end{itemize}

